Multi-Analyst Differential Privacy for Online Query Answering

Most differentially private mechanisms are designed for the use of a single analyst. In reality, however, there are often multiple stakeholders with different and possibly conflicting priorities that must share the same privacy loss budget. This motivates the problem of equitable budget-sharing for multi-analyst differential privacy. Our previous work defined desiderata that any mechanism in this space should satisfy and introduced methods for budget-sharing in the offline case where queries are known in advance. We extend our previous work on multi-analyst differentially private query answering to the case of online query answering, where queries come in one at a time and must be answered without knowledge of the following queries. We demonstrate that the unknown ordering of queries in the online case results in a fundamental limit in the number of queries that can be answered while satisfying the desiderata. In response, we develop two mechanisms, one which satisfies the desiderata in all cases but is subject to the fundamental limitations, and another that randomizes the input order ensuring that existing online query answering mechanisms can satisfy the desiderata.

==> response_letter.tex <==

\begin{center}
    \textbf{Revision Letter: Paper $\# 726$ }
\end{center}

We would like to thank the reviewers for their detailed and insightful comments which have been immensely helpful in the revision process. We have significantly revised our paper in terms of completeness and readability. We have highlighted \new{(in blue)} all new and edited text in the main paper for ease of reference. The following section outlines the changes to the paper.\\ \\

\textbf{Meta-Review}
We have extensively reworked the paper thanks to the feedback of the reviewers. While we leave more detailed comments to each reviewer below we list the larger overall changes here. 
\begin{itemize}
    \item \textbf{R1D1:} We understand that including the theorems in the contributions leads to confusion. We have moved each theorem to their individual section and described them in detail there. 
    
    \item \textbf{R3D2} The proof of \cref{Thrm:SharingIncentiveUpper} (formally Theorem 1) was unclear. We have reworked the theorem to remove the internal lemma which may have caused confusion. Likewise we have included additional information about how the bound of $(\alpha \epsilon/k)^{2/3}$ was derived.
    \item \textbf{R1D3, R3D1:} We have added additional discussion in \cref{Sec:problem} to highlight why the online setting is so fundamentally different than the offline setting.
    \item \textbf{R1D4 : } We have added additional analysis to \cref{sec:motivation} including the classic Laplace mechanism to the experiments.
    \item \textbf{R1D5, R2D3:} We have changed the description of Seeded Cache and Reconstruct along with Algorithm \ref{Algo:SCR} to make it more clear that each analyst goes through the three phases asynchronously depending on their remaining privacy budget. 
    \item \textbf{R1D6, R2D1, R2D2, R3D3 : } We have restructured \cref{experiments} to clarify the experimental design as well as the rationale behind design choices. 
    \item \textbf{R2D5} We have included an additional discussion section at the end  of \cref{experiments} to explain the viability of both seeded cache and reconstruct as well as the query schedulers. This includes a discussion on the additional costs of the query schedulers, namely stalling time.
    \item \textbf{R1D2 :} We have fixed the typos and errors found by the reviewers among others.
\end{itemize}

\textbf{Reviewer 1} 
\begin{itemize}
    \item \textit{ D1: The theorems are duplication and there is no ending mark in some proofs. For instance, Theorem 1,2,3 are put in Introduction Section. Theorem 1 (now \cref{Thrm:SharingIncentiveUpper}) is duplicated in Section 5. Proof of Theorem 1 is in Section 5. Theorem 2,3 (now \cref{Thrm:RandomUniform},\cref{Thrm:RandomGeneral}) are not duplicated in Section 7, but their proofs are included in Section 7.} 
    \begin{itemize}
        \item We have moved each theorem to its appropriate section before their proof. In the introduction section, we have replaced this to forward pointers to the particular theorems.
        \item We have removed the lemma within the proof of \cref{Thrm:SharingIncentiveUpper} (formally Theorem 1). This should make it more clear as to what the ending mark is referring to.
    \end{itemize}
    \item \textit{
D2: Some notations are not explained. For instance, on page 4, The authors wrote: "... tuples (q,i) $\in$ Q×\{1, . . .,k\} consisting of a linear counting
query...". However, $\mathcal{Q}$, q, and i are not explained. In Definition 3,4,5, $\mathbb{E}$ are not explained.}
\begin{itemize}
    \item We have added text clarifying the context of the tuples as a pair of queries and analyst identifiers. Likewise, we have clarified that $\mathbb{E}$ is to denote the expectation over the randomness of the mechanism.
\end{itemize}
\item \textit{D3: Some parts are not explained well. For example, Section1.1 mentions that the online setting is more difficult than the offline one since it has additional constraints. However, these constraints are not explained. The experiment considers 10 analysts and each of them shares the privacy budget e/10. However, the reasons behind this choice are not mentioned.}
\begin{itemize}
    \item We have discussed in more detail some of the prior separations between online and offline query answering including that classes of queries that cannot be answered efficiently in the online setting can be answered in the offline setting. 
    \item We have reworked \cref{experiments} to further describe the design choices for the number of analysts and privacy budget split. We discuss that the choice of 10 analysts is to allow for a diversity of overlapping and disjoint query sequences.
\end{itemize}
\item \textit{D4: Proofs. Theorem 5 (formally Theorem 8) : the proof proves that the error is less than or equal to $\frac{|Q| \sqrt(|Q|)}{e}$ by relying on Theorem 1 (formally theorem 4). However, Theorem 4 proves the privacy budget of DP Composition. It is not clear how Theorem 1 (formally Theorem 4), which does not mention the error, can be used to prove theorem 5(formally Theorem 8.)}
\begin{itemize}
    \item We have further elaborated in \cref{Sec:limitations} on how to derive $\frac{|Q| \sqrt(|Q|)}{\epsilon}$ by showing that splitting the privacy budget $|Q|$ ways and answering each query interdependently. We rely on prior work to get the bound on error. We use \cref{thrm:composoition} (formally theorem 4) to show that this strategy satisfies differential privacy.
\end{itemize}
\item \textit{
The proof of \cref{Thrm:SharingIncentiveUpper} (formally Theorem 1) is very long and should be split into some smaller lemmas. Also, the proof has no ending mark (other proofs have the mark). So it is hard to know which paragraphs belong to the proof.}
\begin{itemize}
    \item The original proof contained the proof mark however it may have been confused for the proof of the additional lemma. As such we have removed the lemma and have directly proved what is now \cref{Thrm:SharingIncentiveUpper} (formally Theorem 1). The proof remains long however that is because the majority of the proof relies on the construction of the two sequences and the expansion to multiple analysts.
\end{itemize}
\item \textit{\cref{Thrm:RandomUniform} (formally Theorem 2) claims that "Any mechanism M which can answer at most c queries with expected error under threshold $\alpha$ with privacy budget $\epsilon$ and can answer at least the first k(log(k)+(c- 1) log(log(k))+O(1)) queries under threshold $\alpha$ with privacy budget $k \cdot \epsilon$ satisfies the sharing incentive." However, the proof does not consider the case of all mechanisms. Instead, it gives a condition that "if a random analyst is chosen at each round...,the expected number of queries required to satisfy the sharing incentive for all analysts is..." .}
\begin{itemize}
    \item we have restated \cref{Thrm:RandomUniform} (formally Theorem 2) as follows : \\ 
        Given a mechanism $M$ which can answer at most $c$ queries with expected error under threshold $\alpha$ with privacy budget $\epsilon$. If a random analyst is chosen at random during each round and if $M$ can answer at least $klog(k)+(c 1) \ log(log(k)+o(1))$ queries with privacy budget $k\epsilon$ then $M$ satisfies the sharing incentive.  \\
        This clarifies the condition in which it satisfies the sharing incentive and implies the use of the randomized scheduler.
\end{itemize}
\item \textit{`The authors claimed that many existing online mechanisms fail to satisfy the sharing incentive or non-interference. However, they only show the failure of one online mechanism, presented in [11], in Section 4.}
\begin{itemize}
    \item In \cref{sec:motivation} we have included additional experiments which also demonstrate that a classic online mechanism, the Laplace mechanism, fails to satisfy the desiderata. 
\end{itemize}
\item \textit{D5. The algorithms are not explained well. Algorithm 1 is not clear since many steps are not explained: line 7, line 12. The sections in the algorithm must be put in its comments and its description. The algorithm's description is also unclear since the lines of the algorithm are not explained. Its variables are also not explained.}
\begin{itemize}
    \item We have revised the descriptions of the algorithms to be more clear. We make it more clear that each analyst goes through the mechanism asynchronously depending on how much privacy budget they have left. Likewise, we've identified in the algorithm box which phase each block of code belongs to. 
\end{itemize}
\item \textit{
D6: Figures in the experiment section do not have x- and y-label. Therefore, it is hard to understand the figures.}
\begin{itemize}
    \item In each of the figures the label of the figure describes which measure is being used for each. To clarify we have included a section that further describes each measure.
\end{itemize}
\end{itemize}


\textbf{Reviewer 2}
\begin{itemize}
    \item \textit{D1. The experimental results are hard to follow, and could do with more interpretation. To a casual reader, the results shown in most plots look quite similar across the different strategies (apart from Ind), and so it is not quite clear what conclusions to draw: is the a significant and consistent difference in behavior to support favoring one method over others? }
    \begin{itemize}
        \item We have added additional explanations as to the difference in mechanism behavior across different $p$ values. Likewise, we have included a discussion section that informs that seeded cache and reconstruct is more stable and should be used in high stakes cases where provably satisfying the desiderata is critical. The query schedulers should be used in cases where some failures can be tolerated. They come with the additional advantage that they can be built on top of the current state of the art.
    \end{itemize}
    \item \textit{D2. For the experiments, time to completion was not clear to me -- where in the paper is this defined? "Time to completion" only appears in Section 8.3.4 and is not explained there. }
    \begin{itemize}
        \item As previously written time to completion was not clear. To clarify we moved it to the end of \cref{sec:measures} and have further elaborated on how it is measured.
    \end{itemize}
    \item \textit{D3. Describing the Cache and Reconstruct algorithm as having 3 phases is a bit confusing, as it implies that each phase happens sequentially, one after another. However, Algorithm 1 clarifies that it is not quite the case: answers are reused when possible, otherwise there is a case split depending on whether the privacy budget is sufficient to answer the given query. The code does not make clear how lambda is determined: is it part of the input, or computed based on other parameters? }
    \begin{itemize}
        \item We recognize this as a point of confusion as such we have altered the description to make it clear that each analyst goes through the phases asynchronously 
        \item We have also adapted Algorithm \ref{Algo:SCR} to further clarify the phases and how each analyst goes through them. This should clarify that the reuse of a query answer only happens in phase 2. 
        \item Likewise, $\lambda$ is left as an input to the mechanism. It should be determined by the data curator based on the accuracy requirement of the problem where higher accuracy requires higher values of $\lambda$
    \end{itemize}
    \item \textit{D4. 
The proof of Lemma 3 (Previously Lemma 4) does not make it very clear what influence the parameters have on this setting: how does lambda need to be set? If lambda is chosen much too large, then there will be no opportunity to construct a basis set of query results. }
\begin{itemize}
    \item It is important to note that seeded cache and reconstruct is analyst monotonic regardless of the choice of the parameters. The basis set is constructed in phase 1 as part of the seed using a fraction of the privacy budget $\gamma$. While it is true that if $\lambda$ is set to be too large no queries will be answered in phase 2 analyst monotonicity is still preserved in this case. \par 
    If phase 2 is skipped entirely then phase 3 will reconstruct queries entirely from the basis created in phase 1. The quality of the basis is entirely dependent on the number of analysts and as such monotonically increases with the increase in analysts. \par 
    While setting $\lambda$ too high will result in no queries being answered in phase 2 the mechanism will still be analyst monotonic. If no queries are answered in phase 2 it remains problematic since a large portion of the privacy budget will be wasted. We have added additional text to clarify regardless of parameter settings.
\end{itemize}

\item \textit{ D5. 
The assumptions behind the results on the query scheduler are not very clear: it seems that one needs to have a set of analysts with a pre-prepared list of queries ready to go. What would happen if (in round robin) we reach an analyst who doesn't have a query right now, but will have some later? It was unclear how to distinguish between round robin, randomized scheduler, and the discounted option of taking a random permutation of queries (the offline case). }
\begin{itemize}
    \item The query schedulers allow for arbitrary online sequences even those where analysts may not have queries ready during their turn. We discuss in \cref{Sec:RandomOrdering} that in the case that a query isn't ready the mechanism stalls and must wait for a query to be ready. This is the additional cost of using the query schedulers and one which we measure in \cref{experiments} as the Time to Completion.
    \item Most online mechanisms ensure some accuracy on the first $n$ queries asked. The query schedulers can be seen as treating those first $n$ queries as a resource and ensuring that each analyst has equal access to that resource. The round robin scheduler does this by ensuring a strict ordering on queries where each analyst is given a turn one at a time. The randomized scheduler however randomizes the order such that in expectation each analyst should receive a similar amount of access to those first queries. \par 
    Randomly permuting queries fails at this goal as analysts who ask a large number of queries will inherently receive larger access to those first, more accurate queries. As such even under a random permutation online mechanisms still fall under the fundamental limit of \cref{Thrm:SharingIncentiveUpper} (formally theorem 1).
\end{itemize}
\end{itemize}




\textbf{Reviewer 3:}
\begin{itemize}
    \item  \textit{D1. This paper follows the multi-analyst differential privacy problem defined in the authors' previous work in [20], in which a mechanism needs to satisfy two properties: sharing incentive and non-interference. This paper extends the offline setting to the online query answering setting. Basically, the authors identify that there is a sharing incentive query limit under the online setting, and present two mechanisms, which are relatively straightforward, to mitigate the problem. I am not sure if the contributions are sufficient to become a new work. }
    \begin{itemize}
        \item We have discussed in more detail how the offline and online settings fundamentally differ in \cref{Sec:problem}. Briefly, the key differences are that there exists classes of queries that can only be answered efficiently in the offline case \cite{OnlineOffline}. Answering these same queries in the online setting incurs significantly more error since they need to be answered one at a time.
        
        In the traditional single analyst case, there is a well known separation between the offline setting and the online setting \cite{OnlineOffline} where specific classes of queries can only be answered in the offline setting. \par 
        In this work, we show that there is a similar clear separation between the online and offline settings when it comes to the sharing incentive. Unlike in the previous separation where specific classes of queries could only be efficient in the offline setting we show that there is a fundamental limit that bounds the number and quality of the queries that can be answered. It is important to note that this bound is polynomial in the number of analysts which is a harsh limit for any online system. \par 
        To address this our paper suggest two possible solutions. Cache and reconstruct which provably satisfies all the desiderata but is subject to this constraint. We also suggest the query schedulers a novel approach for circumventing the constraints by enforcing an ordering of queries in a fair manner. This demonstrates that uniquely in the online case we can adapt existing mechanisms to satisfy the sharing incentive (and keep all of their efficiency) by simply ensuring that each analyst can ask a similar number of queries in the same .

        \item We further discuss the more subtle design choices of cache and reconstruct. Namely that many of the often intuitive practices which increase utility in the single analyst case break the sharing incentive in the multi-analyst case. One of these such changes is the reconstruction of queries. In the single analyst case reconstructing query answers (instead of using privacy budget) whenever the expected error is below $\alpha$ would increase utility. However in the seeded cache and reconstruct the addition of this step would reduce the number of queries in the cache and impact the efficacy of reconstruction on further queries. This leads to cases where the sharing incentive is violated. \par 
        While seeded cache and reconstruct may seem straightforward those steps are chosen precisely how they are to ensure that the cache monotonically increases in size as each analyst joins for all time steps. Ensuring the monotonic increase in the cache is essential to satisfying the sharing incentive and non-interference and selecting steps that optimize while preserving this property is non-trivial.
    \end{itemize}
\item \textit{
    D2. There are several claims that lack explanations.\\
    (1) it is not clear how is the $(\alpha \epsilon / k)^{2/3}$ is derived (above Lemma 3).\\
    (2) the authors claim in Section 5 that "ordering the queries randomly does not circumvent the upper bound of \cref{Thrm:SharingIncentiveUpper} (formally Theorem 1) since the first analyst asks the vast majority of queries". Is it based on the assumption that the number of queries issued by the first analyst is much larger than the other analysts? What if the first analyst only has a small number of queries? Will it change the claim or conclusion?\\
    (3) for the cache and reconstruct mechanism, I wonder, in practice, how many query answers can be reused. It seems the analysts are likely to query with different predicates, which might make this mechanism hard to use. }
    \begin{itemize}
        \item We have added a description in the proof of \cref{Thrm:SharingIncentiveUpper} (formally Theorem 1) which includes the derivation of $(\alpha \epsilon /k)^{2/3}$ from the fundamental lower bounds on error.
        
        \item Since the sharing incentive must hold for any sequence in order to show that the same limit exists in the random order model we need only rely on the same pathological example used in the proof of \cref{Thrm:SharingIncentiveUpper}(formally Theorem 1). In that case, there exists a sequence where the first analyst asks the mass majority of queries while the other $k-1$ analysts ask as little as one query. In that case, the same separation still holds since the first analyst will ask the large majority of the queries prior to any other analyst asking any queries. Likewise in that case the first analyst's query sequence grows with respect to the privacy budget whereas the other analysts' sequences do not. As such, there exists a setting with a very large privacy budget where the first analyst will ask the vast majority of queries first.
        
        \item The number of queries that can be reused in cache and reconstruct is entirely dependent on the similarity of analysts' queries. If in practice the analysts ask queries on disjoint parts of the database with different predicates the amount of resource sharing that can be done is limited. \par 
         It is important to note that since Seeded Cache and Reconstruct satisfies the sharing incentive it can never be worse than independently giving each analyst their share of the privacy budget to answer their own queries.\par 
         In the offline setting where those queries are known in advance, one can construct a single "strategy workload" that can answer all the queries and ensure some sharing of resources even across multiple predicates. In the online case however one can only decide which queries to answer and how to share resources depending on what has already been answered so no universal strategy can be made in that case. This further demonstrates some of the additional complexities that arise specifically in the online case.\par 
         
        Even in the absolute worst case where each analyst has a completely disjoint set of queries to answer they still share budget when creating the initial seed during initialization, therefore, increasing utility with the addition of other analysts. This ensures that not only are analysts ensured a bare minimum utility from the sharing incentive but they still see an increase in utility when they share no queries with other analysts.
        
        
       
    \end{itemize}
    \item \textit{D3. The experimental evaluation section could be further improved.\\
(1) regarding the experimental setting, are there any overlapped queries in the workload? This may give an intuition about to what extent the analysts can reuse the query answers. Also, the authors consider 10 analysts, where the first analyst is chosen with probability p. What about the chosen probabilities of other analysts? It seems there should be a probability vector. I am not sure why here only focuses on the first analyst's probability.\\
(2) Since the proposed mechanisms are general to multiple analysts, would the number of analysts affect the query results, etc.? If so, it may be better to evaluate the effect of the number of analysts, providing more insights. Besides, a set of experiments with respect to different privacy budgets could also give more results for the evaluation.\\
(3) In Figure 3(d)-3(f), it seems the max ratio for different p is quite similar. Is there any reason for this phenomenon? More explanations could be provided to help interpret the experimental results.
}

 \begin{itemize}
        \item The workloads are generated by selecting workloads from a preset set of workloads or generating a randomized workload. These preset workloads contain common workloads that are both asked on the entire database as well as specific predicates. This results in some workloads which contain overlap while other workloads contain no overlap. We have discussed the workload generation in more detail to make that clear. 
        \item We use the $P$ value to demonstrate what happens when a specific analyst under-reports or over-reports queries. Each other analyst is chosen with uniform probability. This allows us to measure the effects of specifically over or under reporting. We have clarified in the writing that each other analyst is chosen with uniform probability. 
        \item We use 10 analysts as a way of showing the impacts of multiple different workloads with possibly competing goals. The impact of adding additional analysts depends on how the privacy budget is distributed. If that analyst joins with additional resources the mechanisms which are analyst monotonic are provably guaranteed to see an increase in utility for each analyst.  \par Alternatively, if an analyst joins without additional resources then the original resources will be spread more thinly across analysts resulting in less utility for each. \par This change in utility with the addition of one analyst (and their resources) is precisely what is measured in the interference.
        \item In these experiments, the max ratio error may look similar at first glance but there are significant differences between the algorithms and how they behave. PMW fails to satisfy the sharing incentive in a majority of changes for any value of $p$ when both analysts are under-represented and over-represented. In cases where analysts are chosen uniformly at random (p=0.1), the max ratio error is significantly less in most cases. For the mechanisms which provably satisfy the sharing incentive, this remains relatively constant regardless of the over/under-representation of particular analysts. we have edited the writing to better reflect this.
    \end{itemize}


\end{itemize}


